Approaches to Conflict-free Replicated Data Types

Conflict-free Replicated Data Types (CRDTs) allow optimistic replication in a principled way. Different replicas can proceed independently, being available even under network partitions, and always converging deterministically: replicas that have received the same updates will have equivalent state, even if received in different orders. After a historical tour of the evolution from sequential data types to CRDTs, we present in detail the two main approaches to CRDTs, operation-based and state-based, including two important variations, the pure operation-based and the delta-state based. Intended as a tutorial for prospective CRDT researchers and designers, it provides solid coverage of the essential concepts, clarifying some misconceptions which frequently occur, but also presents some novel insights gained from considerable experience in designing both specific CRDTs and approaches to CRDTs.

==> mathdefs.tex <==
\RequirePackage{latexsym}
\RequirePackage{dsfont}

% macros for domain teory, semantics, etc. 

% math code definitions

%\mathcode`:="603A          % : as punctuation
%\mathcode`.="613A          % . as punctuation
\mathcode`|="326A          % | as a relation

%\let\es=\relax    %  possible space before punctuation in displayed formulas

%% relations

\newcommand\tx[1]{\hbox{ #1 }}
\newcommand{\defeq}{\stackrel{.}{=}}

\newcommand\vect{\overrightarrow}
\renewcommand\iff{\Leftrightarrow}        % this redefines the original
\renewcommand\implies{\Rightarrow}
\newcommand\implied{\Leftarrow}

\newcommand\sqleq{\sqsubseteq}
\newcommand\sqle{\sqsubset}
\newcommand\sqgeq{\sqsupseteq}
\newcommand\sqgt{\sqsupset}
\newcommand\pleq{\sqleq}          % partial-order leq
\newcommand\ple{\sqle}            % partial-order le
\newcommand\pgeq{\sqgeq}          % partial-order geq
\newcommand\pgt{\sqgt}          % partial-order geq

\newcommand\preleq{\mathrel{%      % pre-order leq
  \raise 2pt\hbox{$\mathop\sqsubset\limits_{\hbox{$\sim$}}$}%
}}

% operators

\newcommand\bigland{\bigwedge}
\newcommand\biglor{\bigvee}

\newcommand\band{\mathbin{\hbox{\&}}}
\newcommand\bor{\mathbin{|}}
\newcommand\bnot{\mathbin{\sim}}

\newcommand\union{\cup}
\newcommand\bigunion{\bigcup}
\newcommand\join{\sqcup}
\newcommand\bigjoin{\bigsqcup}
\newcommand\meet{\sqcap}
%\newcommand\bigmeet{\bigsqcap}
\newcommand\down{\mathord{\downarrow}}
\newcommand\tuple[1]{\mathord{\langle #1 \rangle}}

\newcommand\setsize[1]{\left| #1 \right|}
\newcommand\domxtn{\mathbin{\stackrel{+}{|}}}
\newcommand\domainsub{\mathbin{\lhd\mkern-14mu-}}
\newcommand\domainrestrict[1]{\mathord{|}_{#1}}

% arrows

%\newcommand{\map}{\mathrel{\hookrightarrow}}
\newcommand{\map}{\mathrel{\rightharpoonup}}
\newcommand\goesto[1]{{\mathop{\longrightarrow}\limits^{#1}}}
\newcommand\goes{\longrightarrow}

\newcommand\pfunc{\map}

% function constants

\newcommand\auxfun[1]{\expandafter\newcommand\csname #1\endcsname{%
 \mathop{\hbox{$\mathsf{#1}$}}\nolimits}}
\newcommand\af[1]{\mathop{\hbox{$\mathsf{#1}$}}\nolimits}
\newcommand\kw[1]{\mathrel{\hbox{$\mathbf{#1}$}}}
\newcommand\atom[1]{\mathord{\hbox{\textsc{#1}}}}
\newcommand\field[1]{\mathord{\hbox{$\mathsf{#1}$}}}

\let\max=\relax
\let\min=\relax
\auxfun{max}
\auxfun{min}
\auxfun{dom}
\auxfun{ran}
\auxfun{fst}
\auxfun{snd}

\newcommand\auxrel[1]{\expandafter\newcommand\csname #1\endcsname{%
 \mathrel{\hbox{$\mathsf{#1}$}}}}
\newcommand\rel[1]{\mathop{\hbox{$\mathsf{#1}$}}\nolimits}
\newcommand\arel[1]{\stackrel{\mathsf{#1}}{\longrightarrow}}

% sets

\newcommand{\pow}[1]{\mathcal{P}(#1)}
\newcommand{\mpow}[1]{\mathcal{M}(#1)}

\newcommand{\unit}{\mathds{1}}
\newcommand{\bool}{\mathds{B}}
\newcommand{\nat}{\mathds{N}}
\newcommand{\integer}{\mathds{Z}}
\newcommand{\ids}{\mathds{I}}
\newcommand{\topo}{\mathds{T}}

\newcommand{\false}{\mathsf{False}}
\newcommand{\true}{\mathsf{True}}

\newcommand{\set}{\mathsf{set}}
\newcommand{\poset}{\mathsf{poset}}
\newcommand{\lattice}{\mathsf{lattice}}
\newcommand{\chain}{\mathsf{chain}}
\newcommand{\antichain}{\mathsf{antichain}}



%%%%%%%%%%%

\newcommand\lift[1]{\lfloor #1 \rfloor}

%%%%%%%%%%%%%%%%%%%%%

\newcommand\iffdef{\mathrel{\Longleftrightarrow}}
\newcommand\nullstring{\epsilon}

\newcommand\typeparam[1]{\ensuremath{\langle #1 \rangle}}


